A reduced-order model for segregated fluid-structure interaction solvers based on an ALE approach

This article presents a Galerkin projection-based reduced-order modelling (ROM) approach for segregated fluid-structure interaction (FSI) problems, formulated within an Arbitrary Lagrangian Eulerian (ALE) framework at low Reynolds numbers using the Finite Volume Method (FVM). The ROM is constructed using Proper Orthogonal Decomposition (POD) and incorporates a data-driven technique that combines classical Galerkin projection with radial basis function (RBF) networks. The results demonstrate the numerical stability and accuracy of the proposed method relative to the high-fidelity model. The ROM successfully captures transient flow fields and, importantly, the forces acting on the moving structure without exhibiting unphysical growth or divergence over time. This is further supported by the bounded evolution of error metrics and physical observables, which remain consistent with the full-order simulations throughout the prediction horizon. The method's effectiveness is validated through a benchmark vortex-induced vibration (VIV) case involving a circular cylinder at Reynolds number Re=200. The hybrid ROM approach yields an accurate and efficient tool for solving FSI problems involving mesh motion.

==> sections/NumDiscretization_ijnme.tex <==
\section{Numerical discretization of the full-order and reduced-order models}\label{NumDisFOMROM}
In this section, we recall the details of the  Finite Volumes Method (FVM) in ALE framework, and the reduced form associated.
\subsection{Numerical discretization of the full-order model}\label{standardfv}
The aim of the FVM is to  discretize a system of partial differential equations written in integral form following \cite{moukalled2016finite}. In the present work, a 2-dimensional tessellation is used.  $N_{h}$ will represent the dimension of the full-order model (FOM) which is the number of cells of the discretized problem. 
In the following, the discretization methodology of the momentum and continuity equations will be addressed. In particular, the momentum and continuity equations will be solved using a segregated approach in the spirit of Rhie-Chow interpolation \cite{Rhie1983}. 

To approximate the problem by the use of the FVM, the domain $\Omega = \widehat{\Omega}(t) $ has to be subdivided through a tessellation $\mathcal{T}(t) = \{\Omega_i(t) \}_{i=1}^{N_h}$ so that every cell $\Omega_i(t)$ is a non-convex
polygon and $\bigcup_{i=1}^{N_h} \Omega_i(t) = \Omega (t)$ and $\Omega_i(t) \cap \Omega_j(t) = \emptyset \quad \forall i\neq j$. To simplify the notation, in the following,  $\Omega_i = \Omega_i(t)$ and $S_i = \partial \Omega_i(t)$. Where $S_i$ is the total surface related to cell $\Omega_i$.

We first consider the discretization of the continuity Equation \ref{conteq} in the ALE framework. The finite volumes grid which moves in space must still obey the conservation law as pointed out in Tsui et al. \cite{tsui2013finite}, in which it is stated that as "the change in volume (area) of each control volume between time $t^n$ and $t^{n+1}$  must be equal to the volume (area) swept by the cell's boundary during $\Delta t = t^{n+1} -t^n$", namely
\begin{align}\label{gcl}
\frac{d }{d t}\int_{\Omega_i}d\Omega_i+  \int_{\partial \Omega_i}\boldsymbol{u}^g\cdot \boldsymbol{n} dS= 0.
\end{align}
For every control volume $\Omega_i = \Omega_i(t)$. Here, $\boldsymbol{n}$ is the outward unit normal vector on the boundary surface. The continuity equation written in integral form on control volume $\Omega_i$ reads

\begin{align}\label{eq:continuity_integral}
\frac{d }{d t}\int_{\Omega_i}\rho d\Omega_i+  \int_{\partial \Omega_i} \rho \left(\boldsymbol{u}- \boldsymbol{u}^g\right)\cdot \boldsymbol{n} dS= 0. 
\end{align}
%
Multiplying \cref{gcl} by $\rho$ and making use of the incompressibility constraint yields,
\begin{align}
    \int_{\partial \Omega_i} \boldsymbol{u}^g \cdot \boldsymbol{n} dS = 0
\end{align}
which is the integral version of continuity equation \ref{conteq}, and shows that there is no need to consider the grid velocity in its discretization. 

In the framework of the Finite Volumes Method (FVM), the momentum equation is written in its integral form for every cell of the tessellation
\begin{align}\label{IntegralMomentum}
    \int_{\Omega_i}\frac{\delta \boldsymbol{u}}{\delta t}d\Omega_i + \int_{\Omega_i}\nabla \cdot [\boldsymbol{u}\otimes(\boldsymbol{u} - \boldsymbol{u}_g)]d\Omega_i - \int_{\Omega_i}\nabla \cdot(\mu\nabla \boldsymbol{u})d\Omega_i  + \int_{\Omega_i}\nabla pd\Omega_i = 0.
\end{align}

In the FVM implementation here used, the volume integrals appearing in the momentum equation are computed by means of the so-called \emph{mid-point} quadrature rule. For such a reason, the unknowns of the algebraic problem resulting from the discretization are the values of the unknown fields $\boldsymbol{u}$ and $p$ at the centre of the cells. In particular, we denote with $\boldsymbol{u_i}$ and $p_i$ the velocity and pressure values at the centre of the generic cell $\Omega_i$. 

For a thorough discussion of the FV discretization technique, we refer the interested reader can refer to \cite{ferziger2002computational}. In the next sections,  the numerical treatment of each term in \cref{IntegralMomentum} is analysed and commented.

\subsubsection{The pressure gradient term} 
The pressure gradient term is discretized using Gauss's theorem.
\begin{equation}\label{pressure}
     \int_{\Omega_i}\nabla p d\Omega_i =  \int_{S_i}p d\boldsymbol{S}_i \approx \displaystyle\sum_{j \in S_i}\boldsymbol{S}_{ij}p_{ij}, 
\end{equation} %%$ \boldsymbol{S}_i = \boldsymbol{n} dS_i$
where  $\boldsymbol{S}_{ij}$ is the oriented surface dividing the two neighbour cells $\Omega_i$ and $\Omega_j$, and $p_{ij}$ is the pressure evaluated at the centre of the face $\boldsymbol{S}_{ij}$. Also in the case of surface integrals, we make use of the mid-point quadrature rule.
%Where $\boldsymbol{S}_f$ is the area vector of each face of the control volume and $p_f$ is the value of the pressure at the center of the faces. %see Figure \ref{fig:vp1}. 
\subsubsection{The convective term}
Making once again use of Gauss's theorem, the convective term is discretized as 
\begin{align}
    \int_{\Omega_i}\nabla \cdot [\boldsymbol{u}\otimes(\boldsymbol{u} - \boldsymbol{u}^g)]d\Omega_i  & = \int_{\Omega_i}\nabla \cdot (\boldsymbol{u}\otimes\boldsymbol{u})d\Omega_i - \int_{\Omega_i}\nabla \cdot (\boldsymbol{u}\otimes \boldsymbol{u}^g)d\Omega_i \\
    & = \int_{S_i}d\boldsymbol{S}_i\cdot (\boldsymbol{u} \otimes \boldsymbol{u}) -  \int_{S_i}d\boldsymbol{S}_i\cdot (\boldsymbol{u} \otimes  \boldsymbol{u}^g)\\ 
    &   = \displaystyle\sum_{j \in S_i}\boldsymbol{u}_{ij}F_{ij} - \displaystyle\sum_{j \in S_i}\boldsymbol{u}_{ij}({\boldsymbol{u}^g}_{ij} \cdot \boldsymbol{S}_{ij}) .
\end{align}
%Thanks to the geometrical conservation law stated in  \cref{gcl}.
%With $\boldsymbol{u}_f$   is the velocity vector evaluated at the center of each face of the control volume.
Here,  $\bm{u}_{ij}$ is the velocity evaluated at the centre of the face $\bm{S}_{ij}$, and $F_{ij} = \bm{u}_{ij}\cdot \bm{S}_{ij}$ is the flux of the velocity at the centre of the surface area vector $\bm{S}_{ij}$ sharing the cells $i$ and  $j$ oriented to the cell $j$.
This procedure underlines two considerations. The first one is that $\boldsymbol{u}_{ij}$ is not straightly available, all the variables of the numerical problem are evaluated at the centre of the cells. The values of the variables at the centre of the cell faces must then be obtained based on the values at the cell centres. There are of course several ways to obtain $\boldsymbol{u}_{ij}$ from $\boldsymbol{u}_{i}$. However, the basic idea behind them all is that the face value of each variable is obtained through interpolation of the cell centre values. The second clarification is about the fluxes. During an iterative process for the resolution of the equations, they are calculated using the velocity obtained at the previous step so that the non-linearity involved in such terms is quite naturally treated.
\subsubsection{The diffusion term }
The diffusion term is discretized as follows,
\begin{align}\label{diffusion}
    \int_{\Omega_i}\nabla \cdot  \left( \mu\nabla \boldsymbol{u} \right)d\Omega_i  = \mu_i\int_{S_i}d\boldsymbol{S}_i\cdot  \left( \nabla \boldsymbol{u} \right) \approx \displaystyle\sum_{j \in S_i} \mu_{ij} \boldsymbol{S}_{ij}\cdot (\nabla \boldsymbol{u})_{ij}, 
\end{align}
where $\mu_i$ is the viscosity of the $i-th$ cell, $\mu_{ij}$ is the viscosity evaluated at the centre of $\bm{S}_{ij}$, and $(\nabla \boldsymbol{u})_{ij}$ is the gradient of $\boldsymbol{u}_{ij}$ evaluated at the centre of $\bm{S}_{ij}$. 
As for the evaluation of the term $\boldsymbol{S}_{ij}\cdot (\nabla \boldsymbol{u})_{ij}$ in \cref{diffusion}, it involves the --- unknown --- gradient of the velocity at the face of the cell. Also in this case, we resort to interpolation to obtain such gradient. 
For orthogonal meshes,   the term  $\boldsymbol{S}_{ij}\cdot (\nabla \boldsymbol{u})_{ij}$ is computed as
\begin{align}\label{orthogonal-mesh}
\boldsymbol{S}_{ij}\cdot (\nabla \boldsymbol{u})_{ij} \approx 
\|\boldsymbol{S}_{ij}\|
\frac{\boldsymbol{u}_i- \boldsymbol{u}_j}{\|\boldsymbol{d}_{ij}\|}, 
\end{align}
where $\boldsymbol{d}_{ij}$ represents the vector connecting the centres of cells of index $i$ and $j$. We recall that a mesh is orthogonal if the line that connects two neighbouring cell centres is orthogonal to the face that divides the two cells. 

With non-orthogonal grids, the one-dimensional interpolation in \cref{orthogonal-mesh} loses accuracy, as the face centre is not lying on the line connecting the neighbouring cell centres. Thus, a correction term has to be added, and the interpolation corrected for non-orthogonality \cite{jasak1996error} reads
\begin{align}\label{non-orthogonal-mesh}
    \boldsymbol{S}_{ij}\cdot (\nabla \boldsymbol{u})_{ij} = \|\boldsymbol{\pi}_{ij}\|\frac{\boldsymbol{u}_i-\boldsymbol{u}_j}{\|\boldsymbol{d}\|} + \boldsymbol{k}_{ij} \cdot (\nabla \boldsymbol{u})_{ij}.
\end{align}
Herein, $\boldsymbol{S}_{ij} = \boldsymbol{\pi}_{ij} + \boldsymbol{k}_{ij}$ and  $\boldsymbol{\pi}_{ij}$ is chosen to be parallel to $\boldsymbol{S}_{ij}$ and $\boldsymbol{k}_{ij}$ to be orthogonal to $\boldsymbol{d}$. The term $(\nabla \boldsymbol{u})_{ij}$ is obtained through interpolation of the values of the gradient at the cell centres $(\nabla \boldsymbol{u})_i$ and $(\nabla \boldsymbol{u})_j$. 

\subsubsection{The PIMPLE algorithm}

Based on the aforementioned considerations, the discretized form of \cref{momentum} and  \cref{conteq} is written in the following matrix form
\begin{equation}\label{compactmatform}
    \left[ 
       \begin{array}{cc}
         \mathbf{A}_u   & \mathbf{B}_p  \\
           \nabla (\cdot) & \mathbf{0}
       \end{array}
       \right]
    \left[ 
       \begin{array}{c}
         \boldsymbol{u}_h \\
           \boldsymbol{p}_h
       \end{array}
\right]  =  \mathbf{0},
%\left[ 
%\begin{array}{c}
%\mathbf{0}\\
%0
%\end{array}
%\right].
\end{equation}
where $ \boldsymbol{u}_h$ and $\boldsymbol{p}_h$ being the vectors where all $\boldsymbol{u}_i$  and  $p_i$ variables are collected respectively. With $\boldsymbol{u}_h \in \mathbb{R}^{dN_h}$ and $\boldsymbol{p}_h \in \mathbb{R}^{N_h}$.  ${N_h}$ is the number of cells in the mesh,  and  $d$ the  spacial dimension of the problem. Additionally, $\mathbf{A}_u$  is the matrix containing the terms related to velocity for the discretized momentum equation, $\mathbf{B}_p$ the matrix containing the terms related to pressure for the same equation, and $ \nabla (\cdot)$ the matrix representing the incompressibility constraint operator. The system matrix in \cref{compactmatform} has a saddle point structure which is usually difficult to invert using a coupled approach. For this reason, in this work we make use of a segregated approach, in which the momentum equation is solved with a tentative pressure and later corrected by exploiting the divergence-free constraint.


The segregated approach used in this work is based on the PIMPLE algorithm implemented in the OpenFOAM library \cite{jasak2007openfoam}. PIMPLE algorithm is a  mix of SIMPLE \cite{patankar1983calculation}, and  PISO \cite{issa1986solution} algorithms, and is mostly suitable for unsteady problems requiring high Courant number and/or dynamic mesh setups such as the one considered in this study.  

% Other approaches to deal with geometrically parametrized problems that do not use a dynamic mesh are also possible. These methods relied on full-order immersed formulations. The interested reader might refer to \cite{ZengStabileKaratzasScovazziRozza2022, KaratzasStabileNouveauScovazziRozza2019a, KaratzasStabileNouveauScovazziRozza2019b} for more details. 
We here report a brief description of the PIMPLE algorithm. In particular, we mainly focus on the aspects that most affect the resolution of the online problem in the ROM strategy proposed in this work. 

As with the SIMPLE algorithm, PIMPLE is an iterative strategy that, at each time step, aims at converging to the correct pressure and velocity fields --- i.e. the ones respecting the continuity constraint. At each iteration, the first sub-step carried out is that of solving the discretized momentum equation, in which the pressure field is the one obtained at the previous iteration.  
In the following,  $\boldsymbol{u}_h^{n*}$ denotes the velocity which does not necessarily satisfy the continuity equation, while $\boldsymbol{u}_h^{n}$ does. 
The momentum matrix is divided into diagonal $\mathbf{A}$ and extra-diagonal parts $\mathbf{H}(\cdot)$
\begin{equation}\label{MomemtumMatrix}
  \mathbf{A}_u   \boldsymbol{u}_h^{n*} = \mathbf{A}\boldsymbol{u}_h^{n*} -  \mathbf{H}(\boldsymbol{u}_h^{n*}),
\end{equation}
with $n$ being an index to identify a generic iteration and $ \mathbf{A}_u$ satisfying the following relation 
\begin{align}\label{MomentumPredictor}
\mathbf{A}_u   \boldsymbol{u}_h^{n*} = -\mathbf{B}_p\boldsymbol{p}_h^{n-1}. 
\end{align}
By using \cref{MomemtumMatrix}, the momentum equation can be reshaped as follows
\begin{align}\label{velstar}
   \mathbf{A}\boldsymbol{u}_h^{n*} = \mathbf{H}(\boldsymbol{u}_h^{n*}) - \mathbf{B}_p\boldsymbol{p}_h^{n*} \Rightarrow & \boldsymbol{u}_h^{n*} =  \mathbf{A}^{-1}\mathbf{H}(\boldsymbol{u}_h^{n*})- \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}_h^{n-1}.
\end{align}
In a further iterative \textit{inner loop} small corrections to the velocity and pressure fields is introduced as
\begin{align}\label{corrections}
  \boldsymbol{u}_h^n = \boldsymbol{u}_h^{n*} + \boldsymbol{u}'  ~~~~~~~~~~ \boldsymbol{p}_h^n = \boldsymbol{p}_h^{n-1} + \boldsymbol{p}'.
\end{align}
The symbol $'$ denotes the corrections for both terms.
Inserting \cref{corrections} in \cref{velstar}, and rearranging terms yields
\begin{equation}\label{Mixterms}
   \boldsymbol{u}_h^n - \boldsymbol{u}' = \mathbf{A}^{-1}[\mathbf{H}(\boldsymbol{u}_h^{n}) - \mathbf{H}(\boldsymbol{u'})-\mathbf{B}_p\boldsymbol{p}_h^{n}+\mathbf{B}_p\boldsymbol{p}'].
\end{equation}
From \cref{Mixterms}, it is possible to deduce a relation between $\boldsymbol{u}'$ and $\boldsymbol{p}'$
\begin{equation}\label{uprime}
    \boldsymbol{u}' = \Tilde{\boldsymbol{u}}' - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}', 
\end{equation}
with 
\begin{equation}\label{utildeprime}
    \Tilde{\boldsymbol{u}}' = \mathbf{A}^{-1}\mathbf{H}(\boldsymbol{u}').
\end{equation}
As the following relation holds thanks to \cref{MomentumPredictor} :
\begin{align}
\bm{u}_h^n = 
\mathbf{A}^{-1}[ \mathbf{H}(\bm{u}_h^{n}) -\mathbf{B}_p\boldsymbol{p}_h^{n} ].
\end{align}
With the use of \cref{uprime} and the divergence operator $\nabla (\cdot)$ applied to $\boldsymbol{u}_h^{n}$ in \cref{corrections} knowing $\boldsymbol{u}'$ from \cref{uprime},  one obtain an equation that directly relates $\boldsymbol{p}'$ and $\boldsymbol{u}_h^{n*}$:
\begin{equation}
    [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'\right) = [\nabla (\cdot)]\boldsymbol{u}_h^{n*} + [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'.
\end{equation}
Which is basically the discretized Poisson equation for pressure (PPE) expressed in terms of the velocity and pressure corrections.
%With some approximations for the mixed terms, the following holds:
%\begin{eqnarray}
% \boldsymbol{u}_h^n =    \mathbf{A}^{-1}\left[\mathbf{H}(\boldsymbol{u}_h^{n*}) + \mathbf{H}(\boldsymbol{u}')- \mathbf{B}_p\boldsymbol{p}_h^{n-1} - \mathbf{B}_p\boldsymbol{p}' \right].
%\end{eqnarray}
In the SIMPLE algorithm, the velocity correction $\Tilde{\boldsymbol{u}}'$ is unknown as $\mathbf{H}(\boldsymbol{u}')$, hence neglected implying the following relation:  
\begin{equation}\label{relvelstarandpprime}
    [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'\right) = [\nabla (\cdot)]\boldsymbol{u}_h^{n*}.
\end{equation}
Therefore, $\boldsymbol{p}'$ is expressed as the only function of $\boldsymbol{u}_h^{n*}$ in \cref{relvelstarandpprime}. Then the corrected pressure is entered again in \cref{velstar} in order to obtain a new velocity field $\boldsymbol{u}_h^{n*}$ and repeat the procedure until the pressure correction falls below a given \textit{tolerance} and the velocity satisfy both the continuity and momentum equation. 

As the $\Tilde{\boldsymbol{u}}'$ is neglected, the SIMPLE algorithm converges slowly and is used mainly for steady-state simulations. Furthermore, to avoid instabilities, relaxation factor $\alpha_p$ and $\alpha_u$ are introduced in the computation of $\boldsymbol{p}_h^{n}$ and $\boldsymbol{u}_h^{n*}$ as follows:
\begin{align}
   &  \boldsymbol{p}_h^{n}  = \boldsymbol{p}_h^{n-1} + \alpha_p\boldsymbol{p}',\\
   & \boldsymbol{u}_h^{n*}  =  \mathbf{A}^{-1}\mathbf{H}(\boldsymbol{u}_h^{n*})- \alpha_u \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}_h^{n-1}.
\end{align}
%a big assumption is taken since the extra-diagonal term $\mathbf{H}(\boldsymbol{u}')$ is neglected and put to zero. 
%Eventually, this makes the whole procedure no more consistent, but in the meantime, it makes the resolution of the so-called pressure correction step much easier. We then get:
%\begin{equation}
%    \boldsymbol{u}_h =    \mathbf{A}^{-1}\left[\mathbf{H}(\boldsymbol{u}_h^{n-1}) - \mathbf{B}_p\boldsymbol{p}_h^{n}  \right].
%\end{equation}
%By applying the divergence operator to both sides of Equation \ref{}, we obtained the Poisson equation for pressure thanks to the incompressibility constraint:
%\begin{align}
%    [\nabla (\cdot)] \boldsymbol{u}_h = [\nabla (\cdot)] \left( \mathbf{A}^{-1}\left[\mathbf{H}(\boldsymbol{u}_h^{n-1}) - \mathbf{B}_p\boldsymbol{p}_h^{n}  \right] \right)  %\Rightarrow & [\nabla (\cdot)]\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}_h^{n} = [\nabla (\cdot)]\mathbf{H}(\boldsymbol{u}_h^{n-1})
%\end{align}

The PISO algorithm comes to play to speed up the convergence after neglecting $\Tilde{\boldsymbol{u}}'$ and \textit{computing the pressure correction}  $\boldsymbol{p}'$  using \cref{uprime}. $\boldsymbol{u}'$ is  computed  as follows:
\begin{equation}\label{1stpresscorr}
    \boldsymbol{u}' = - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'.
\end{equation}
Allowing the computation of $\Tilde{\boldsymbol{u}}'$ using \cref{utildeprime}. One defines a second velocity correction equation mirroring \cref{uprime} as follows:
\begin{equation}\label{PISO}
    \boldsymbol{u}'' = \Tilde{\boldsymbol{u}}' - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''. 
\end{equation}
As $\boldsymbol{u}''$ in \cref{PISO} satisfy the continuity equation, one define  also a second pressure correction equation as:
\begin{equation}\label{2ndpresscorr}
      [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'' \right) =   [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'.
\end{equation}
%In summary,  what basically  the PISO algorithm makes more compared to the SIMPLE algorithm to add an inner loop to correct the pressure and velocity a second time. 
To sum up, what the PISO algorithm does more than the SIMPLE algorithm is to add a second inner loop to correct pressure and velocity. This speeds up the convergence, allowing this algorithm to be used in a transient simulation.  Following the procedure described by \cref{1stpresscorr,PISO,2ndpresscorr} further corrections steps can be  added, increasing both the algorithm's convergence and computational cost. 



\subsection{Rigid body motion and mesh motion strategy}\label{motionstrategies}
%The mesh motion technique considered here is a 
In the resolution algorithm, the vertical displacement of the cylinder is accounted for by interfacing the fluid solver with Newton’s second law \cref{ode} for the rigid cylinder, written in the global inertial reference frame. Such a second-order ODE is in this work solved using the Symplectic 2nd-order explicit time-integrator for solid-body motion \cite{dullweber1997symplectic}.
% \begin{align}
%     \displaystyle\sum \boldsymbol{F} & = m \boldsymbol{a}, \label{Newton2law}\\
%     \displaystyle\sum \boldsymbol{M} & = \boldsymbol{\alpha}\boldsymbol{I}. \label{Newton2law2}
% \end{align} %%In order to calculate the motion of the body we need to know the acceleration
% where $\boldsymbol{a}$ and $\boldsymbol{\alpha}$ are respectively  the linear and angular accelerations of the system. In addition, $m$ denotes the body mass, $\boldsymbol{I}$ the inertia.   $\boldsymbol{F}$ and  $\boldsymbol{M}$ are the combined forces and  moments present in the system. 
% In  FSI simulations, $\boldsymbol{F}$ can include contributions from the viscous and pressure forces exerted by the fluid on the body, and forces due to mechanical elements such as springs or dampers.  
After the linear displacement and velocity of the cylinder have been computed, the position of the cylinder boundary and the corresponding Dirichlet boundary datum for the velocity are updated in the fluid dynamic solver. Of course, due to rigid body kinematics consideration, the velocity prescribed on the cylinder boundary is uniform and equal to the velocity obtained solving \cref{ode}. To complete the interface between the structural --- rigid body --- solver and the fluid dynamic solver, the fluid grid must be updated to adjust to the boundary nodes motion while preserving good cells quality. 
 
In this work, the mesh deformation technique used is the so-called Slerp (Spherical Linear Interpolation) given its capability of deforming volumetric grids in presence of --- translational and rotational --- rigid boundary motions \cite{jasak2007openfoam}. For some alternatives to the mentioned mesh motion strategy, the interested reader may refer to \cite{MM2016, Jasak2007AutomaticMM, deBoer2007} and to references therein for more details. Finally, a finite difference scheme is used to obtain the grid velocity field $\boldsymbol{u}^g$ from the computed grid deformation field. 



Finally, the essential steps of the PIMPLE algorithm combined  mesh motion strategy described in this section are reported in \cref{alg:pimple}.  In  \cref{alg:pimple},  the iterations within one time-steps are called \textit{outer iterations}, they are performed in an \textit{outer loop} in which the structural problem is solved, the cylinder position and the fluid mesh are updated, along with the coefficients and the source matrix of the discretized equations. The operations performed on linear systems with fixed coefficients are called instead \textit{inner iterations} and they occur in the so-called \textit{inner loop}.
\begin{algorithm}[h]
\caption{PIMPLE algorithm with dynamic mesh.}\label{alg:pimple}
\begin{algorithmic}
\Require{\text{Initial fields $\boldsymbol{u}_h^{n*}$, $\boldsymbol{p}_h^{n-1}$, and $\boldsymbol{\delta}^0$}  \Comment{$\boldsymbol{\delta}^0$ is the initial node displacement};} 
\While{ $t \leq t_{end}$ }
      \While{$\text{No. outer corrections $\geq$ 2}  ~~ \text{and} ~~\text{Tol} \geq \text{maxTol} $}
          \State Compute the forces; \Comment{Using $\boldsymbol{u}_h^{n*}$, $\boldsymbol{p}_h^{n-1}$}\;
          \State Solve the rigid body problem \cref{ode}  \Comment{To obtain the new cylinder's position}\;
          \State Solve the mesh motion problem \Comment{To obtain $\boldsymbol{\delta}^n$ }\;
          \State $\mathbf{A}_u \boldsymbol{u}_h^{n*}$  \Comment{Assembling the momentum matrix \cref{MomemtumMatrix}}\;
         \State  Solve $\mathbf{A}_u \boldsymbol{u}_h^{n*} = -\mathbf{B}_p\boldsymbol{p}_h^{n-1}$  \Comment{Momentum predictor \cref{MomentumPredictor} to obtain $\boldsymbol{u}_h^{n*}$}\;
         \State $ [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'\right) = [\nabla (\cdot)]\boldsymbol{u}_h^{n*}$ \Comment{Assembling the matrix of PPE \cref{relvelstarandpprime}}\;
          \State Solve $ [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'\right) = [\nabla (\cdot)]\boldsymbol{u}_h^{n*}$ \Comment{PPE to obtain $\boldsymbol{p}'$} \;
          \State $\boldsymbol{u}' \gets - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'$\Comment{ Momentum corrector \cref{1stpresscorr}} \;
          \While{$ \text{No. inner corrections }$ } 
              \State $[\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''\right) = [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'$  \Comment{Assembling the matrix for PPE  
                \cref{2ndpresscorr}}\;
              \State Solve $ [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''\right) = [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'$ \Comment{Recursively to obtain $\boldsymbol{p}''$}\;
              \State $\boldsymbol{u}' \gets \Tilde{\boldsymbol{u}}' - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''$: \Comment{Momentum corrector \cref{PISO}} \;
          \EndWhile
              \State $\boldsymbol{u}_h^{n*} \gets \boldsymbol{u}'$ \;
              \State $\boldsymbol{p}_h^{n-1}\gets \boldsymbol{p}_h^{n-1} + \boldsymbol{p}'$ \;
       \EndWhile
\EndWhile
\Ensure{\text{$\boldsymbol{u}_h^{n}$, $\boldsymbol{p}_h^{n}$, and $\boldsymbol{\delta}^n$;}}
\end{algorithmic}
\end{algorithm}

\subsection{The reduced-order problem}\label{rompro}
In this section, we recall the details of the proper orthogonal decomposition, the concept of  POD-Galerkin projection,  and POD-Interpolation (POD-RBF) using radial basis networks.
\subsubsection{The Proper orthogonal decomposition}\label{POD}
The Proper Orthogonal Decomposition (POD) is used to construct the low-dimensional space. The POD is a compression technique where a set of numerical realizations (in time or parameter space) is reduced into a number of orthogonal basis (spatial modes) that capture the essential information suitably combined from previously acquired system data \cite{anttonen2005applications}. 
%\gs{the sentence above is not really writtein. What does it mean a compressed method? Maybe a compression technique?}

This work applies the POD to a group of realizations called snapshots. It consists of computing a certain number of full-order solutions $\bm{s}_i = \bm{s}(t_i)$ where $t_i \in \bm{T}$ for $i = 1, \cdots, N$. $\bm{T}$ being the training collection of a certain number $N$ of the time values, to obtain a maximum amount of information from this costly stage to be employed later on for a cheaper resolution of the problem. Those snapshots can be assembled at the end of the resolution into a so-called \emph{snapshot matrix} $\boldsymbol{S} \in \mathbb{R}^{N_h\times N}$ defined as
\begin{align}
    \boldsymbol{S} & = \left[\boldsymbol{s} (\boldsymbol{x},t_1), \dots, \boldsymbol{s} (\bm{x},t_{N}) \right].
\end{align}
The idea is to compute the ROM solution that can minimize the error denoted here by $E^{ROM}$ see \cref{Erom} between
the obtained realization of the problem and its high-fidelity counterpart. 
In the POD-Galerkin scheme, the reduced-order solution is represented as 
\begin{align}\label{seqq}
\boldsymbol{s} (\boldsymbol{x},t) \approx  \boldsymbol{s}^{ROM} (\boldsymbol{x},t) = \displaystyle\sum_{i=1}^{N_r}a_i(t)\boldsymbol{\phi}_i(\boldsymbol{x}).
\end{align}
Where $N_r \ll N_h$ ($N_h$ is the number of cells in the computational domain) is a predefined number,  $\boldsymbol{\phi}_i$ is a generic pre-calculated orthonormal function depending only on the space while $a_i(t)$ is the temporal modal coefficients  satisfying the conditions  
\begin{align}
    & a_j(t)  =   \left(\boldsymbol{\phi}_j,  \boldsymbol{s} (\boldsymbol{x},t) \right)_{L^2 (\Omega)},
    %& \left<a_i(t) a_j(t) \right>   = \frac{1}{T}\int_{0}^{T} a_i(t) a_j(t)dt =  \lambda_i \delta_{ij}.
    & \boldsymbol{\phi}_j^{\intercal} \bm{M} \boldsymbol{\phi}_i = \bm{\delta}_{ij}.
\end{align}
$\bm{M}$ being  the mass matrix defined by the chosen inner product. In the case of $L^2$-norm and FVM $\bm{M}$ is a diagonal matrix containing the cell volumes. 
The best performing functions $\boldsymbol{\phi}_i$ in this case, are  the ones minimizing the  $L^2$-norm error $E$ between all the reduced-order solutions $\boldsymbol{s}^{ROM}_i$, $i = 1, \cdots, N$ and their high fidelity counterparts, namely
\begin{align}\label{Erom}
    E = \displaystyle\sum_{i=1}^{N}\|\boldsymbol{s}^{ROM}_i - \boldsymbol{s}_i\|_{L^2(\Omega)} =  \displaystyle\sum_{i=1}^{N}\|\boldsymbol{s}_i - \displaystyle\sum_{i=1}^{N_r}\left(\boldsymbol{s}_i, \boldsymbol{\phi}_i\right)_{L^2(\Omega)}\boldsymbol{\phi}_i \|_{L^2(\Omega (t_0))}.
\end{align}
$\Omega (t_0)$ being the reference configuration of the computational domain in the case of grid motion. Note that the projection is performed with respect to $L^2(\Omega(t))$ while POD is computed with respect  to $L^2(\Omega(t_0))$. 
It can be shown \cite{Kunisch2002} that solving a minimization problem based on \cref{Erom} is equivalent to solving the eigenvalue problem 
\begin{align}\label{eigenproblem}
    \boldsymbol{C} \mathbf{V} = \mathbf{V}\boldsymbol{\lambda}.
\end{align}
 $\boldsymbol{C} \in \mathbb{R}^{N\times N}$ being the correlation matrix between all the different training solutions of the snapshot matrix $\boldsymbol{S}$, $\mathbf{V} \in \mathbb{R}^{N\times N}$ is the matrix whose columns are the eigenvectors, and $\boldsymbol{\lambda} \in \mathbb{R}^{N\times N}$  is a diagonal matrix whose diagonal entries are the eigenvalues.  The entries of the correlation matrix are defined as follows
\begin{align}\label{correlation}
\boldsymbol{C}_{ij} = \left(\boldsymbol{s}_i, \boldsymbol{s}_j \right)_{L^2\Omega (t_0))},
\end{align}
using a POD strategy, the required basis functions are obtained through the resolution of the eigenproblem mentioned in \cref{eigenproblem}, obtained with the method of snapshots by solving \cref{Erom}. The required basis functions  are then computed from the eigenvalues and eigenvectors in \cref{eigenproblem} as 
\begin{eqnarray}
    \boldsymbol{\phi}_i = \displaystyle\dfrac{1}{N\sqrt{\lambda_i}}\displaystyle\sum_{j=1}^{N}\boldsymbol{s}_jV_{ji} ~~~~~ \forall i = 1, \cdots, N.
\end{eqnarray}
All the basis functions are collected into a single matrix:
\begin{equation}
      \boldsymbol{\Phi} = \left[\boldsymbol{\phi}_1, \cdots, \boldsymbol{\phi}_{N_r} \right] \in \mathbb{R}^{N_h \times N_r}.
\end{equation}
Which is used to project the high fidelity problem onto the reduced subspace so that the final system dimension is $N_r$. 
In the framework of ROM analysis, the \emph{offline phase} consists in carrying out multiple resolutions of the FOM problem, collecting the snapshots to assemble the snapshot matrix, computing the modes through eigenproblem \cref{eigenproblem}, and projecting the FOM problem onto the reduces subspace. Once this computationally expensive phase is done, the procedure results in a solution system (the \emph{online phase}) characterized by a small amount of unknowns, and by computational cost that is much lower than the original problem. In the next sections, we will provide details on the way we adapted the Galerkin projection procedure to the present fluid-structure interaction application.

\subsubsection{Reduced-PIMPLE algorithm for incompressible laminar flows}\label{sectredpimple}
This part assumed that the  high fidelity  model is discretized and written in the  form    
%The full-order model for both the velocity and pressure in the discretized form  is given by:
\begin{align}\label{discritizefullmodel}
\mathbf{A}_u \boldsymbol{u}_h = \boldsymbol{b}_u,  ~~~~~~	\mathbf{B}_p \boldsymbol{p}_h = \boldsymbol{b}_p.
\end{align}
With $\mathbf{A}_u \in \mathbb{R}^{dN_h\times dN_h}$, $\boldsymbol{u}_h \in \mathbb{R}^{dN_h}$, $\mathbf{B}_p \in \mathbb{R}^{N_h\times N_h}$, $\boldsymbol{p}_h \in \mathbb{R}^{N_h}$, $\boldsymbol{b}_u \in \mathbb{R}^{N_h}$,  and $\boldsymbol{b}_p \in \mathbb{R}^{N_h}$ are  defined  in \cref{compactmatform}.  
As already mentioned, $N_h$ is the number of control volumes (cells) in the mesh, and $d=2$ is the space dimension. 
%Now, the Galerkin projection is used for the construction of the low-dimensional space. 
The following equation introduces the resulting reduced model expansions of the velocity and pressure fields respectively
$\boldsymbol{u}_h (\boldsymbol{x},t) \approx \boldsymbol{u}_r (\boldsymbol{x},t)$ and $\boldsymbol{p}_h(\boldsymbol{x},t) \approx p_r(\boldsymbol{x},t)$, with
\begin{align}\label{ueqq}
\boldsymbol{u}_r (\boldsymbol{x},t) =  \displaystyle\sum_{i=1}^{N_u}a_i(t)\boldsymbol{\phi}_i(\boldsymbol{x}) = \boldsymbol{\Phi} \boldsymbol{a}^{\intercal},~~~~~ p_r(\boldsymbol{x},t) = \displaystyle\sum_{i=1}^{N_p}b_i(t)\boldsymbol{\xi}_i(\boldsymbol{x}) = \boldsymbol{\Xi} \boldsymbol{b}^{\intercal}.
\end{align}
Herein,  $a_i(t)$,  and  $b_i(t)$ are temporal modal coefficients;  $\boldsymbol{\phi}_i$ and $\boldsymbol{\xi}_i$ are the basis functions of POD modes of the velocity and pressure fields stored  respectively in $\boldsymbol{\Phi} \in \mathbb{R}^{dN_h\times N_u}$ and $\boldsymbol{\Xi} \in \mathbb{R}^{N_h\times N_p}$ with $N_u$ and $N_p$ being the numbers of basis functions selected for the prediction of the velocity and pressure solutions respectively.  $\boldsymbol{a} \in \mathbb{R}^{N_u}$ and $\boldsymbol{b} \in \mathbb{R}^{N_p}$ are  the vectors containing the temporal coefficients for the velocity and pressure, respectively.  
We point out that for the construction of the reduced basis spaces, the POD strategy discussed in \cref{rompro} is used on the snapshot matrices of the velocity and pressure fields separately, in order to obtain two different families of reduced basis functions.
\begin{align}\label{basismatrices}
\boldsymbol{\Phi}= \left[\boldsymbol{\phi}_1,\dots, \boldsymbol{\phi}_{N_u} \right] \in \mathbb{R}^{dN_h\times N_u}, ~~~~~~
\boldsymbol{\Xi} = \left[\boldsymbol{\xi}_1, \dots, \boldsymbol{\xi}_{N_p} \right] \in \mathbb{R}^{N_h\times N_p}.
\end{align}
The linear systems in \cref{discritizefullmodel} are projected respectively into the low-dimensional using in \cref{basismatrices}. Thus, the following relation holds: 
\begin{align}\label{redsystems}
 \boldsymbol{A}_u^r\boldsymbol{a} = \boldsymbol{b}_u^r, ~~~~~~~~~~~~~~~~  \boldsymbol{A}_p^r\boldsymbol{b} = \boldsymbol{b}_p^r.
\end{align}
Where $\boldsymbol{A}_u^r = \boldsymbol{\Phi}^{\intercal}\mathbf{A}_u\boldsymbol{\Phi} \in \mathbb{R}^{N_r^u\times N_r^u}$,    $\boldsymbol{A}_p^r = \boldsymbol{\Xi}^{\intercal}\mathbf{A}_p\boldsymbol{\Xi} \in \mathbb{R}^{N_r^p\times N_r^p}$, $\boldsymbol{b}_u^r = \boldsymbol{\Phi}^{\intercal}\boldsymbol{b}_u \in \mathbb{R}^{N_r^u}$, and $\boldsymbol{b}_p^r = \boldsymbol{\Xi}^{\intercal}\boldsymbol{b}_p \in \mathbb{R}^{N_r^p}$.
The resulting systems in \cref{redsystems} can be solved using any method for dense matrices. In this work, we used the Householder rank-revealing QR decomposition of a matrix with full pivoting implemented in the Eigen library \cite{eigenweb}. The whole idea here is to rely on a method capable of being as coherent as possible with respect to the high-fidelity \cref{alg:pimple} discussed earlier. The main steps of the reduced algorithm
for incompressible laminar flows are summarized in \cref{alg:redpimple}. We point out that in the current version of the algorithm, steps 7 and 10 have to be carried out on the full order grid, with a consequent impact on the reduced order model computational cost. 

\begin{algorithm}[h]
\caption{Reduced-PIMPLE algorithm with dynamic mesh}\label{alg:redpimple}
\begin{algorithmic}
\Require{$\boldsymbol{u}_h^{n*}$, $\boldsymbol{p}_h^{n-1}$, $\boldsymbol{\delta}^0$, $\boldsymbol{\Phi}$, $\bm{\Psi}$, and $\boldsymbol{\Xi}$;}
\While{ $t \leq t_{end}$ }
      \While{$\text{No. outer corrections $\geq$ 2}  ~~ \text{and} ~~\text{Tol} \geq \text{maxTol} $}
          \State Compute the forces; \Comment{Using $\boldsymbol{u}_h^{n*}$, $\boldsymbol{p}_h^{n-1}$}\;
          \State Solve the rigid body problem \cref{ode}  \Comment{To obtain the new cylinder's position $y^C_{new}$}\;
           \State Compute $\boldsymbol{c} = RBF (y^C_{new})$ \cref{rbfnns}\;
          \State Reconstruct ${\bm{\delta}}^n  = \bm{\Psi}^{\intercal} \boldsymbol{c}$ \cref{POD_displacements}\;
           \State $\mathbf{A}_u \boldsymbol{u}_h^{n*}  = \mathbf{b}_u$ \Comment{Assembling the momentum matrix \cref{MomentumPredictor}}\;
          \State  Solve $\boldsymbol{\Phi}^{\intercal} \mathbf{A}_u \boldsymbol{\Phi} \boldsymbol{a}^{*} =\boldsymbol{\Phi}^{\intercal} \mathbf{b}_u$ \Comment{To obtain $\boldsymbol{a}^{*}$ \text{with} $\mathbf{b}_u =-\mathbf{B}_p\boldsymbol{p}_h^{n-1}$} \;
           \State Reconstruct $\boldsymbol{u}_h^{n*}$\  \Comment{Using $\boldsymbol{a}^{*}$}\;
          \State $ [\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'\right) = [\nabla (\cdot)]\boldsymbol{u}_h^{n*}$\Comment{Assembling the matrix of PPE \cref{relvelstarandpprime}}\;
           \State Solve $\boldsymbol{\Xi}^{\intercal} \mathbf{A}_p \boldsymbol{\Xi} \boldsymbol{b}' = \boldsymbol{\Xi}^{\intercal}\boldsymbol{b}_p$ \Comment{To obtain $\boldsymbol{b}'$}\;
          \State Reconstruct $\boldsymbol{p}'$\  \Comment{Using $\boldsymbol{b}'$}\;
         \State $\boldsymbol{u}' \gets - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}'$ \Comment{Momentum corrector \cref{1stpresscorr}} \;
          \While{\text{No. inner corrections } } 
               \State $[\nabla (\cdot)]\left(\mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''\right) = [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'$  \Comment{Assembling the matrix for PPE  
                \cref{2ndpresscorr}}\;
               \State Solve $\boldsymbol{\Xi}^{\intercal} \mathbf{A}_p \boldsymbol{\Xi} \boldsymbol{b}'' = \boldsymbol{\Xi}^{\intercal}\boldsymbol{b}_p$ \  \Comment{Recursively to obtain $\boldsymbol{b}''$ \text{where} $\boldsymbol{b}_p = [\nabla (\cdot)]\Tilde{\boldsymbol{u}}'$}\;
               \State Reconstruct $\boldsymbol{p}''$\  \Comment{Using $\boldsymbol{b}''$}\;
              \State  $\boldsymbol{u}' \gets \Tilde{\boldsymbol{u}}' - \mathbf{A}^{-1}\mathbf{B}_p\boldsymbol{p}''$: \Comment{Momentum corrector \cref{PISO}} \;
           \EndWhile
            \State $\boldsymbol{u}_h^{n*} \gets \boldsymbol{u}'$ \;
            \State $\boldsymbol{p}_h^{n-1}\gets \boldsymbol{p}_h^{n-1} + \boldsymbol{p}'$ \;
       \EndWhile
\EndWhile
    \Ensure{\text{ $\boldsymbol{u}_h^{n}$, $\boldsymbol{p}_h^{n}$, and $\boldsymbol{\delta}^n$;}}
\end{algorithmic}
\end{algorithm}

\subsubsection{POD with interpolation for mesh motion prediction}\label{pod-i}
This section presents a method to reduce the computational cost associated with the mesh motion part in the system. Along with a reduction of resolution system degrees of freedom, the advantage of this methodology is to make the online equations independent of the specific equations solved at the full order levels to compute the mesh deformation. As will be discussed,  the methodology combines proper orthogonal decomposition with radial basis functions (RBF) networks applied to the grid nodes displacement field.  
% Taking the known points $\boldsymbol{x}_k$ to be the centers of the radial basis functions and evaluating the values of the basis functions at the same points.  

So, the first step of the mesh deformation reduction strategy is that of computing the POD modes of the grid nodes displacement field. To this end, we assemble a snapshot matrix with the grid nodes displacements obtained at different time steps

\begin{align}
    \boldsymbol{S}^g & = \left[\boldsymbol{d}^g (\boldsymbol{x},t_1), \dots, \boldsymbol{d}^g (\boldsymbol{x},t_{N}) \right].
\end{align}
As in the case of pressure and velocity unknowns, the matrix $\boldsymbol{S}^g$ is then processed to obtain a correlation matrix using \cref{correlation} and, from the solution of an eigenvalue problem as in \cref{eigenproblem}, a set of POD modes. The reduced-order solution for the grid displacement field is then represented as, 
\begin{align}\label{POD_displacements}
\boldsymbol{d}^g (\boldsymbol{x},t) \approx   \displaystyle\sum_{i=1}^{N_r^d}c_i(t)\boldsymbol{\psi}_i(\boldsymbol{x}),
\end{align}
%
where $N_r^d$ is the amount of modes considered for the grid displacement field. Along with the modal functions $\boldsymbol{\chi}_i(\boldsymbol{x})$, the solution of eigenvalue \cref{eigenproblem} provides the values of the modal coefficients in correspondence with each time step included in the snapshot matrix. For such a reason, a natural choice for computing the grid deformation at time instants not included in the snapshots would be that of interpolating the modal coefficients based on the time variable. However, given the fact that the grid nodes displacement is induced by the --- rigid --- translation of the cylinder boundary $y^C$, a more meaningful way to obtain the modal coefficients at each time step is to consider that
\begin{equation}
c_i(t)=\widehat{c}_i(y^C(t))\quad i=1,\dots,N_r^d,    
\end{equation}
and interpolate the $c_i$ values based on the cylinder vertical displacement variable --- as obtained at each of the time steps at which the solution snapshots have been collected.

In this work, the interpolation step of the data driven POD strategy used for the reduction of the grid nodes displacement field is carried out by means of the Radial Basis Function \cite{LAZZARO2002521} method. In the present framework, modal coefficient $c_i$ at a generic value $y^C$ is obtained evaluating the expression
\begin{equation}\label{rbfnns}
    c_i(y^C)  = \displaystyle\sum_{k=1}^{N}w_k\rho(|| y^C - y^C_k ||), 
\end{equation}
in which $\rho:\mathbb{R}\rightarrow\mathbb{R}$ is in the so-called \emph{radial basis}.  $\rho$ is a function of the Euclidean distance. In the present case it is a one dimensional function, but in more general cases it maps the $m$ dimensional parameter space in $\mathbb{R}$. The weights $w_k$ appearing in \cref{rbfnns} are determined imposing the interpolation condition at the snapshots, in which the modal coefficients are known from \cref{eigenproblem}. The conditions used are then

\begin{equation}\label{rbfnns_colloc}
    (c_i)_j=c_i(y^C_j)  = \displaystyle\sum_{k=1}^{N}w_k\rho(|| y_j^C - y^C_k ||) \quad j=1,\dots,N 
\end{equation}
resulting in the system
 \begin{equation}\label{rbfweights}
   \boldsymbol{c}   = \mathbf{G} \boldsymbol{w}^{\intercal}, 
 \end{equation}
in which $ \mathbf{G} = (g_{kj}) = \rho(|| y_j^C - y^C_k ||)$ is the Gram matrix. So, once the weights have been computed solving system \eqref{rbfweights} in the offline phase, in the online computations the modal coefficients are obtained evaluating \cref{rbfnns}.

We point out that, despite in the present case the $c_i$ coefficients only depend on a scalar variable, in the case of multidimensional dependence, RBF interpolation can be used with no algorithmic modifications. Thus, more complex cases in which the cylinder exhibits rigid motions with more translational and rotational degrees of freedoms, could still be treated with the methodology described. Even in the case in which the FSI problem involves a deformable body which alters the shape of one or more boundaries of the fluid domain, RBF 
could be still used to interpolate the fluid mesh nodal displacements based on the structural displacements reduced coefficients. 

Finally, we remark that the RBF interpolation can also be interpreted as a network in which $N$ is the number of neurons in the hidden layer, $y^C_k$ is the centre vector for neuron $k$, $\boldsymbol{w}_k$ being the weight of neuron $k$ in the linear output neuron. Given this analogy, we point out that different and more efficient networks can substitute RBF --- which has a $O(N^2)$ computational cost --- in future works.


%The RBF  is used to interpolate a map $f: \mathbb{R} \mapsto \mathbb{R}$  known at some finite number of points $f(\boldsymbol{x}_k) = y_k$, $k = 1, \cdots, N$. $\rho$ is a given basis function of the Euclidean distance, $N$ is the number of neurons in the hidden layer, $\boldsymbol{x}_k$ is the center vector for neuron $k$, and $\boldsymbol{w}_j$ being the weight of neuron $j$ in the linear output neuron %\cref{rbfnns} can be rewritten as a linear system, namely:
% \begin{equation}\label{rbfweights}
%   \boldsymbol{y}   = \mathbf{G} \boldsymbol{w}^T, 
% \end{equation}
% where $ \mathbf{G} = (g_{kj}) = \rho(||\boldsymbol{x}_k - \boldsymbol{x}_j ||)$ being the Gram matrix. The weights are given by: $\boldsymbol{w} = \mathbf{G}^{-1}\boldsymbol{y}$.
%The rationale behind POD-RBF regards the evaluation of the new %temporal or parameterized coefficients 
%computed at the parameter points $\vartheta_k$; in this case, %it will be the cylinder's position  at a given time t. 
%Next, the separability's assumption on the point displacement %field is given as follows:
%\begin{equation}\label{POD-displacement}
%    \boldsymbol{\delta} ( \boldsymbol{x}, t_k )  \approx \displaystyle\sum_{i=1}^{N_{\delta}}c_i(\vartheta (t_k))\boldsymbol{\psi}_i(\boldsymbol{x}), ~~~  \forall \vartheta (t_k)=\vartheta_k \in \Theta.
%\end{equation}
%$\Theta$ being the training set of the airfoil motion at the %offline stage, and $N_{\delta}$ the require number of basis to %approximate the $\boldsymbol{\delta}$. 
%In the online stage, as input, a new time-parameter value %$\vartheta_{new}$ is given,  and using the trained weights %obtained from \cref{rbfweights},  the coefficient $c_i =  %c_i(\vartheta_{new})$ is obtained by interpolation with RBF %and $\vartheta_{new}$ is obtained by solving  \cref{ode} at %the online stage. Then, the new coefficient is computed by:
%\begin{equation}\label{ThetaNew}
%    c (\vartheta_{new}) =  \displaystyle\sum_{j=1}^{N_{\delta}}\boldsymbol{w}_j\rho(||\vartheta_{new} - \vartheta_j ||).
%\end{equation}
%The new point displacement is predicted as follows:
%\begin{equation}\label{pod-rbfs}
%    \boldsymbol{\delta} (\boldsymbol{x}, t_{new})  = \displaystyle\sum_{i=1}^{N_{\delta}}c_i(\vartheta_{new} )\boldsymbol{\psi}_i(\boldsymbol{x}) =  \Psi \boldsymbol{c}^T.
%\end{equation}
% \subsection{POD-Interpolation}\label{pod-i}
% This section presents a method to reduce the computational cost associated with the mesh motion part in the system. The methodology combines POD and RBF networks on the point displacement field. RBF networks can be used to interpolate a function $f: \mathbb{R} \mapsto \mathbb{R}$
% when the values of this function are known on the finite number of points $f(x_k) = v_k$, $k = 1, \cdots, N$.  Taking the known points $x_k$ to be the centers of the radial basis functions and evaluating the values of the basis functions at the same points.  The interpolation using RBF functions is based on the following formula: 
% \begin{equation}\label{rbfnns}
%     f(x_j)  = \displaystyle\sum_{j=1}^{N}w_j\rho(||x_j -x_k ||), 
% \end{equation}
% where $\rho$ is a given basis function of the Euclidean distance, $N$ is the number of neurons in the hidden layer, $x_k$ is the center vector for neuron $k$, and $w_j$ is the weight of neuron $j$ in the linear output neuron. Equation \ref{rbfnns} can be rewritten as a linear system, namely:
%  \begin{equation}
%    \boldsymbol{v}   = \mathbf{G} \boldsymbol{w}^T, 
%  \end{equation}
%  where $ \mathbf{G} = g_{kj} = \rho(||x_k - x_j ||)$. The weights can be obtained from the equation
%  \begin{equation}
%      \boldsymbol{w} = \mathbf{G}^{-1}\boldsymbol{v}.
%  \end{equation}
% The rationale behind POD-RBF regards the evaluation of the POD coefficients by interpolating the POD coefficients computed for the parameter points (in this case, it will be the transverse displacement of the cylinder at a given time t) $\theta_k \in \Theta$. $\Theta$ is the training set of the cylinder displacement at the offline stage. 
% By using the POD assumption, the linear decomposition of the point displacement field is written as follows:
% \begin{equation}
%     y ( \boldsymbol{x}, \theta_k (t) )  \approx \displaystyle\sum_{i=1}^{N_d}c_i(\theta_k (t))\xi_i(\boldsymbol{x}),  ~~~~~ \forall \theta_k \in \Theta  .
% \end{equation}
% In the online stage, as input, a new time-parameter vector $\theta^{*}$ is given,  and using RBF,  the coefficient $c_i =  c_i(\theta^{*})$ is  obtained by interpolation with RBF and $\theta^{*}$ is obtained by solving Equation \ref{ode} at the online stage. Then, the new coefficient is computed by:
% \begin{equation}
%     c (\theta^{*}) =  \displaystyle\sum_{j=1}^{N_{par}}w_j\rho(||\theta^{*} -\theta_j ||).
%     %RBF(\theta_{k+1} (t) )
% \end{equation}
% And the point displacement is reconstructed following:
% \begin{equation}
%     y (\boldsymbol{x}, \theta^{*})  = \displaystyle\sum_{i=1}^{N_d}c_i(\theta^{*} (t) )\xi_i(\boldsymbol{x}).
% \end{equation}
% POD, in combination with a radial basis function (RBF) interpolation network which can determine interpolation coefficients, can accurately reproduce
% dimensional aspects, boundary conditions, and/or material properties as they apply to the system or model \cite{ashley2018application}. The application of POD-RBF interpolation can reduce the model's dimensionality and reproduce the unknown field corresponding to any arbitrary set of parameters $\Theta$. It can be noticed that POD projection and interpolation share the exact eigenfunctions and distinguish each other by the method to obtain amplitudes \cite{wang2012comparative}. The POD interpolation method calculates amplitudes by interpolating scattered data, while the POD projection method calculates amplitudes by projecting continuous governing equations onto the low dimensional space spanned by eigenfunctions.  It is worth mentioning that both methods have their advantages and disadvantages.


